GliDe with a CaPE: A Low-Hassle Method to Accelerate Speculative Decoding

Speculative decoding is a relatively new decoding framework that leverages small and efficient draft models to reduce the latency of LLMs. In this study, we introduce GliDe and CaPE, two low-hassle modifications to vanilla speculative decoding to further improve the decoding speed of a frozen LLM. Specifically, GliDe is a modified draft model architecture that reuses the cached keys and values from the target LLM, while CaPE is a proposal expansion method that uses the draft model's confidence scores to help select additional candidate tokens for verification. Extensive experiments on different benchmarks demonstrate that our proposed GliDe draft model significantly reduces the expected decoding latency. Additional evaluation using walltime reveals that GliDe can accelerate Vicuna models up to 2.17x and further extend the improvement to 2.61x with CaPE. We will release our code, data, and the trained draft models.

==> icml2024/chapter/1_intro.tex <==
\section{Introduction}

% \jjcomment{In general, you need to cite more papers in this section to support your claims.}
% \cxdu{ok prof, I wanna add the citation after the draft.}
With Large Language Models~(LLMs) becoming more and more powerful, they are now extensively applied in people's daily lives. 
Examples include both general-purpose LLMs (such as ChatGPT and Claude) and domain-specific models (such as Copilot for coding and DriveGPT4 for autonomous driving).
The improvement in LLMs' capabilities is largely attributed to the increased model capacity, which called the scaling laws of LLMs.
However, as models grow in size, the costs associated with training and inference have also largely increased, which is not desirable. 
In particular, during inference, prolonged latency would significantly affect user experience. 
Therefore, accelerating LLMs' inference process is a critical issue to be addressed.

The key issue lies in LLM inference is the memory-bounded behavior caused by autoregressive nature. 
Different from training where the batch size is large, the batch size of inference is highly variable and often much smaller, frequently reduced to one in some cases like the edge device.  This small batch presents unique challenges in optimizing inference efficiency due to its IO-bounded nature. Distinguishing it significantly from the batch-oriented optimization strategies commonly employed during the training phase.

To overcome the bottleneck of IO, several classic techniques have been proposed, such as MoE, pruning, and the recent method called speculative decoding. Unlike other approaches, speculative decoding can achieve lossless acceleration. Its fundamental idea involves employing a small language model (SLM) to predict the next $n$ tokens, followed by a larger model that runs in parallel to validate these tokens. Due to the IO-bounded nature of the process, the larger model can verify $n$ tokens in a parallel manner, often at the same speed as generating a single token. Furthermore, based on [specific theory], it is demonstrated that speculative greedy decoding/sampling is consistently equivalent to LLM greedy decoding/sampling in terms of results.

\jjcomment{To quickly get to the key idea of this paper, I'd suggest using just one paragraph (instead of the three paragraphs above) to introduce speculative decoding and its importance.}
\cxdu{ok prof.}

Unfortunately, speculative decoding is not always guaranteed to speed up. According to the formula proposed in [specific theory] $speedup = \frac{1 - \alpha^{k+1}}{(1-\alpha)(kc + 1)}$, we can calculate the expected speed-up ratio as shown in Figure 1. 
The formula implies the two factors of the small model affecting the acceleration: the acceptance rate and the computation overhead of the small model.
The computation overhead of small models $c$ is inversely proportional to the speed-up ratio, while the acceptance rate of small models $\alpha$ is proportional to the speed-up ratio.
According to the scaling law, the fitting capability of small models is constrained by the number of parameters directly linked to the computation overhead indicating a trade-off between the two factors.

However, please note our task is not to build an independent small language model, but rather a proposer language model to assist the LLM. These two different tasks have distinct requirements for the design of small models, which is an aspect previously overlooked in prior research. In our work, we re-examine the role of the small language model in speculative decoding. We find the following special characteristics for the speculative small language model: 1) Since the LLM has to verify tokens, the SLM can access the information of the verified tokens from the LLM. 2) The SLM can scarify the output accuracy for speed because the role of the SLM is to be a good proposer and the bad output will be corrected by the LLM. and 3) The SLM does not need to propose only one output, and it can generate multiple outputs (fragments) for better acceptance. 

Considering these three features, we design the SLM specifically for speculative decoding. Firstly, inspired by the encoder-decoder architecture, we can utilize the LLM as a special \textit{encoder} to enhance the representational ability of the SLM. Specifically, we reuse the last $l$ layers of KV cache from the large model as an additional input to the SLM. After each self-attention layer in the SLM, we insert a cross-attention module to facilitate interaction between the current representations of the SLM and the LLM.  The input keys and values of this layer are from the LLM's KV cache and the queries are from  SLM itself.  This approach offers two primary benefits: First, due to its larger number of parameters and deeper layers, an LLM is generally believed to possess more abstract and high-level representations, as demonstrated in probing tasks xx. Second, as we stated earlier, the large model inherently computes the previous inputs during the verification phase, with the results being cached in the GPU as the key-value (KV) Cache. Thus, the \textit{encoder} itself does not require additional time to run. We call this model \textbf{GL}impse \textbf{S}LM (\textbf{GLS}). The computation and storage of KV cache is more like a free lunch for SLM.  Compared to the vanilla speculative decoding, the only increase in computational load is attributed to the lightweight cross attention layer in the GLS which is about 0.33x of the whole model. Additionally, our method requires the same GPU memory as the vanilla model.

For the second point, different from an independent SLM, the output of the SLM in speculative decoding will be corrected by the LLM. This implies that our SLM can sacrifice a portion of its generation quality (acceptance rate) in exchange for reduced its own costs. This is because the speed-up ratio is determined jointly by both the two factors, and the speculative decoding framework ensures that the output of the model remains unchanged.
 Consider an extreme case where we use an LLM as the SLM. In this scenario, its acceptance could reach 100\%, but since the cost of running the SLM is equivalent to that of the LLM, this approach would result in at least double the time consumption. To find the best architecture of SLM we examine the scaling law between different sizes of SLMs and their acceptance rate for different LLMs. Different from previous studies using deep SLM like Llama-160m which has 12 layers, our experiments suggest that the SLM should be shallower. Although a shallower SLM leads to a decrease in acceptance, the acceleration in runtime due to reduced layers is more significant. Additionally, we find that increasing the hidden size of SLM can effectively compensate for the decrease in acceptance rate caused by reducing the number of layers, but with much less time cost. Therefore, we suggest using a shallower and wider SLM for speculative decoding.


% may not good corresponded to the third points
Lastly, we also focus on whether the acceptance of SLM is predictable. We find that the output distribution confidence of  SLM is highly positively correlated with the average number of tokens accepted by LLM. And due to the SLM is not required to generate a fix number proposal, we decide to use this finding to further expand the proposal without runing the SLM multiple times like beam search. We develope a new proposal expansion method for the SLM called \textbf{C}onfidence-\textbf{A}ware \textbf{P}refix \textbf{E}xpansion decoding (\textbf{CAPE}) to further increase the number of accepted tokens when the batch size is low.

\paragraph{Contributions} Our main contributions are as follows:
\begin{itemize}
    \item Addressing the collaborative working pattern of speculative decoding, we propose a specially small language model named \textbf{GL}impse \textbf{S}LM (\textbf{GLS}). GLS is capable of better inference by glimpse the key-value (KV) cache of the LLM. Moreover, to further enhance the acceleration effect, we also conduct the scaling law of the size of the GLS.
    \item We also design a Confidence-\textsc{a}ware Prefix Expansion (\textsc{CaPE}) algorithm, which is simple but largely improves the acceptance under low batch size inference settings.
    \item We applied our GLS to two different architectures of mainstream Large Language Models, Vicuna (7B, 13B, 33B) and Mistral (7B), across five public datasets. Compared to the standard speculative decoding, our method demonstrated significant improvements across all datasets. In practical tests on mt-bench, our method GLS-\textsc{CaPE} achieved at least a 2.2x speedup. Our code and SLMs will be released.
\end{itemize}

==> icml2024/chapter/backup/oldcape.tex <==
\iffalse

\begin{table}[htbp]
\centering
\caption{The comparison between our cape and other proposal expansion methods, where adaptive refers to whether it can make a different number of proposals for different samples.}
\label{tab: compare cape}
\begin{tabular}{@{}lccc@{}} % 
\toprule
Method & Base Model(s) &Execution(s)& Adaptive \\ % table head
\midrule
Medusa & NAR & 1 &  $\times$ \\
Beam Search & AR & Beam size & $\times$ \\
% Specinf & ARs & ARs count & $\times$ \\
\textsc{CaPE} (ours) & AR & 1 & \checkmark \\
\bottomrule
\end{tabular}
\end{table}



\jjcomment{I will revise the motivation for CAPE later.}

In the original speculative decoding, at each speculation step, the draft model proposes a single sequence of $\gamma$ tokens for the target model to verify.
Some recent work explored the idea of generating multiple proposed sequences at a single speculation step for the target model to concurrently verify.
Representative methods include SpecInfer~\cite{miao2023specinfer} and Medusa~\cite{medusa2023}.
However, SpecInfer requires multiple draft models.
Medusa essentially uses a non-autoregressive draft model to speculate next tokens in different positions and considers all combinations of them to form multiple sequences. 
Because the speculated tokens at different positions are generated separately, they may not form fluent sequences when combined together, an issue similar to what non-autoregressive translation faces~\cite{NAT, Du2021OAXE}.
In this paper, we propose a simple alternative method that uses the standard single, auto-regressive draft model to form multiple proposals.

% \cxdu{Hi prof, you can also have a glimpse at the following. except for confidence, these methods are also requires multiple drafters or non-autoregressive drafters.}

Previous works~\cite{miao2023specinfer, medusa2023} propose let the draft model generate multiple outputs and use tree attention to do parallel verification.
However, ~\citet{miao2023specinfer} requires multiple distributed draft models and ~\citet{medusa2023} use a non-autoregressive (NAR) draft model which can output multiple outputs at once.
Then the challenge of single autoregressive (AR) draft model is how to generate multiple outputs, and beam search is a valid but not wise choice.
Because beam search is very time-consuming due to the sort and copy operation. 
We introduce our proposed \textsc{CaPE} here to avoid previous mentioned challenge by the following two advantages:
1) Zero additional execution and 2) Confidence-aware expansion.

\textsc{CaPE} only does prefix expansion, which means it will first run the draft model as without \textsc{CaPE}. And then collect each time output distribution to do prefix expansion as Figure.~\ref{fig:cape} shows: the original output's prefix ``\textit{is all}" can be expanded to ``\textit{is all you}". This prefix expansion add \textbf{zero} additional execution of the draft model.

Let $x_{\leq t}$ denote the prefix or prompt passed to the draft model during the current round of speculation.
For each position $n \in [t+1, t+\gamma]$, let $x^*_n$ denote the token that is predicted by the draft model to have the highest probability at that position.
Let $\mathcal{X}_n$ denote the set of top-ranked tokens at position $n$.

During the subsequent verification step, we pass the sequence $(x^*_{t+1}, x^*_{t+2}, \ldots, x^*_{t+\gamma})$ to the target model for parallel verification.

Let $x^*_k$ denote the first token in the sequence that fails the verification.
In standard speculative decoding, the target model will generate the correct token $x_k$ at this position based on its next token distribution.
In CAPE, in addition to generating this token $x_k$, the target model can generate one more token $x_{k+1}$ as long as $x_k$ is in $\mathcal{X}_k$.




In our further investigation of speculative decoding, we find there exist a positive correlation between the output confidence of draft model (i.e., the maximum value of the prediction distribution) and the acceptance rate. As shown in Figure~\ref{fig: confacc}, we sample approximately 6 million tokens to analyze the relationship between output confidence and acceptance rate. It is evident that higher confidence corresponds to a higher acceptance rate.

We aim to leverage this characteristic to enhance the acceptance rate. So we do a confidence-aware prefix expansion here. 
As the Figure~\ref{fig:cape} third step shows, when the distribution's confidence is lower, we include more words in the proposal (i.e., the red tokens). We set a 10 bins array $C$ for the confidence from the range of 0.0 to 0.9, and the proposal words are equal to $C[round(max(p)*10)]$ for each step confidence $max(p)$. In our experiments, we set $C$ as $[8,8,8, 6, 6, 6, 4, 4, 2, 2]$.

Unlike Medusa does cartesian product expansion, \textsc{CaPE} only expands on the prefix. This primarily has two reasons: 
(1) Unlike Medusa's non-autoregressive nature, GLIDE is an autoregressive model. This means that subsequent tokens are conditional on the results of previous predictions. A Cartesian product would link incorrect errors of prefixes and successors. 
(2) Although the expansion set of prefix expansion is a subset of the Cartesian product's expansion set, compared to the Cartesian product, prefix expansion significantly reduces the tokens that need verification by the  target model. This means that \textsc{CaPE} can be extended to batch-serving scenarios in future work.


\jjcomment{My description of CAPE starts from here.}
\fi


\ignore{
Because the success of SD relies much on both the quality and the efficiency of the draft model, how to design an effective draft model becomes an important research question.
Since SD was first proposed, there have been several studies proposing better draft models.
One idea is to make the draft model align better with the target model (e.g., DistilSpec~\cite{zhou2024distillspec}).
However, existing work has not fully taken advantage of the hidden representations in the target model during the draft model's speculation stage.
We hypothesize that by leveraging the KV cache of the target model, the draft model can generate the speculated tokens that align better with the target model's distributions.
We therefore propose a novel architecture for the draft model that uses cross-attention to attend to the KV cache of the target model and thus improve its predictive power.
We also observe that the draft model's confidence scores have a high correlation with the acceptance rate. 
This motivated us to design a conference-aware prefix expansion mechanism, in which the draft model generates multiple proposals sharing a common prefix.
When the target model verifies these different proposals concurrently, it is almost always able to verify one more token compared with standard speculative decoding with a single proposal.
This improves the acceptance rate and reduces the running time of speculative decoding.
}

==> icml2024/table/main_exp_table.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lr cc cc cc cc}
\toprule
\multirow{2}{*}{\bf ~~~~~~~~~Models} & \multirow{2}{*}{\bf Cost} & \multicolumn{2}{c}{\textbf{GSM8K}} & \multicolumn{2}{c}{\textbf{Fin.-Alp.}} & \multicolumn{2}{c}{\textbf{Spider}} & \multicolumn{2}{c}{\textbf{Code-Py.}} \\
 \cmidrule(lr){3-4}\cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
 &$\downarrow(\%)$ &Acc. \footnotesize{(\%)} &$\mathbb{E}$(Spd.) 
&Acc. \footnotesize{(\%)} &$\mathbb{E}$(Spd.)
&Acc. \footnotesize{(\%)}&$\mathbb{E}$(Spd.)
&Acc. \footnotesize{(\%)}&$\mathbb{E}$(Spd.)\\
\midrule
 $\mathcal{M}_{T}$:~\textbf{Vicuna-7B}\\
~~~~~~~~~\footnotesize{\textsc{LLaMA}-68m} &7.7 &51.6 &1.46 &49.7 &1.41 &19.2 &0.89 &34.8 &1.11\\
\footnotesize{$\mathcal{M}_{D}$~~\textsc{LLaMA}-160m} &49.0 &58.0 &0.66 &57.1 &0.65 &25.1 &0.38 &40.0 &0.48 \\
~~~~~~~~~\footnotesize{\textsc{GliDe}-47m} & \bf 6.7  &~~\textbf{64.8}$^{\dagger}$ &~~\textbf{1.97}$^{\dagger}$ &~~\textbf{63.2}$^{\dagger}$ &~~\textbf{1.90}$^{\dagger}$ &~~\textbf{55.7}$^{\dagger}$ &~~\textbf{1.64}$^{\dagger}$ &~~\textbf{67.0}$^{\dagger}$&~~\textbf{2.06}$^{\dagger}$ \\
\midrule
 $\mathcal{M}_{T}$:~\textbf{Vicuna-13B}\\
~~~~~~~~~\footnotesize{\textsc{LLaMA}-68m} &6.2 &50.2 &1.51 &49.3 &1.48 &19.0 &0.94 &32.7 &1.13\\
\footnotesize{$\mathcal{M}_{D}$~~\textsc{LLaMA}-160m} &39.3 &56.8 &0.75 &56.8 &0.75 &25.4 &0.45 &38.3 &0.54 \\
~~~~~~~~~\footnotesize{\textsc{GliDe}-47m} & \bf 5.5 &~~\textbf{67.1}$^{\dagger}$ &~~\textbf{2.16}$^{\dagger}$ &~~\textbf{65.0}$^{\dagger}$ &~~\textbf{2.07}$^{\dagger}$ &~~\textbf{57.1}$^{\dagger}$ &~~\textbf{1.77}$^{\dagger}$ &~~\textbf{68.6}$^{\dagger}$ 
&~~\textbf{2.24}$^{\dagger}$  \\
\midrule
 $\mathcal{M}_{T}$:\textbf{Vicuna-33B}\\
~~~~~~~~~\footnotesize{\textsc{LLaMA}-68m} &4.6 &49.1 &1.57 &46.5 &1.50 &30.0 &1.16 &31.5 &1.19\\
\footnotesize{$\mathcal{M}_{D}$~~\textsc{LLaMA}-160m} &29.5 &56.1 &0.89 &53.1 &0.84 &31.4 &0.59 &36.7 &0.64 \\
% vanilla is 66m
~~~~~~~~~\footnotesize{\textsc{GliDe}-71m} & \bf 6.8 
&~~\textbf{69.3}$^{\dagger}$  &~~\textbf{2.16}$^{\dagger}$  
&~~\textbf{64.3}$^{\dagger}$  &~~\textbf{1.94}$^{\dagger}$  
&~~\textbf{62.7}$^{\dagger}$  &~~\textbf{1.87}$^{\dagger}$  
&~~\textbf{68.9}$^{\dagger}$ &~~\textbf{2.14}$^{\dagger}$  \\
\midrule
 \multicolumn{4}{l}{$\mathcal{M}_{T}$:~\textbf{Mistral-7B-Instruct}}\\
\footnotesize{$\mathcal{M}_{D}$~~}\footnotesize{\textsc{LLaMA}-45m}$^{*}$ &4.9 &36.7 &1.27 &40.2 &1.34 &41.9 &1.38 &44.5 &1.44 \\
~~~~~~~~~\footnotesize{\textsc{GliDe}-47m} &  \bf 6.6 &~~\textbf{60.1}$^{\dagger}$  &~~\textbf{1.80}$^{\dagger}$  &~~\textbf{56.4}$^{\dagger}$  &~~\textbf{1.67}$^{\dagger}$  &~~\textbf{59.8}$^{\dagger}$  &~~\textbf{1.79}$^{\dagger}$  &~~\textbf{62.6}$^{\dagger}$  &~~\textbf{1.89}$^{\dagger}$ \\
\bottomrule
\end{tabular}
\caption{Comparisons of the acceptance rate (Acc.) and expected speedup $\mathbb{E}$(Spd.) of \textsc{GliDe} and previous draft models from ~\citet{miao2023specinfer}.  $^\dagger$ denotes significantly better than the best \textsc{LLaMA} draft models with $p<0.01$.
\textbf{Cost} denotes the walltime between the draft model and target model once running.
*Since there is no open-source draft model implemented for mistral, we retrained it using the same data of \textsc{GliDe}.
The only difference with \textsc{GliDe} is the removal of cross attention. }
\label{tab:main}
\end{table*}
